Divide and Scale: Formalization and Roadmap to Robust Sharding

Sharding distributed ledgers is a promising on-chain solution for scaling blockchains but lacks formal grounds, nurturing skepticism on whether such complex systems can scale blockchains securely. We fill this gap by introducing the first formal framework as well as a roadmap to robust sharding. In particular, we first define the properties sharded distributed ledgers should fulfill. We build upon and extend the Bitcoin backbone protocol by defining consistency and scalability. Consistency encompasses the need for atomic execution of cross-shard transactions to preserve safety, whereas scalability encapsulates the speedup a sharded system can gain in comparison to a non-sharded system. Using our model, we explore the limitations of sharding. We show that a sharded ledger with $n$ participants cannot scale under a fully adaptive adversary, but it can scale up to $m$ shards where $n=c'm\log m$, under an epoch-adaptive adversary; the constant $c'$ encompasses the trade-off between security and scalability. This is possible only if the sharded ledgers create succinct proofs of the valid state updates at every epoch. We leverage our results to identify the sufficient components for robust sharding, which we incorporate in a protocol abstraction termed Divide & Scale. To demonstrate the power of our framework, we analyze the most prominent sharded blockchains (Elastico, Monoxide, OmniLedger, RapidChain) and pinpoint where they fail to meet the desired properties.

==> 5comparison.tex <==
\section{Evaluation of sharding protocols}\label{app:comaprison} 
We evaluate existing sharding protocols with respect to the desired properties defined in Section \ref{subsec:ledger}. In particular, we analyze \el, \mx, \ol, and \rc, and discuss \cs. The analysis can be found in Appendix~\ref{sec:eval}, while the summary of our evaluation can be found below and is illustrated in Table~\ref{tab:comparison}. 
% In the following, we present a summary of our evaluation for each protocol; we begin with the overview of each protocol and we include only the critical components to pinpoint where each protocol fails. 


\begin{table*}[ht]
\vspace{-0.2cm}
    \centering
 \caption{Summarizing sharding protocol properties under our model}
\begin{tabular}{l|cccccc}
        \toprule
                     \text{Protocol}              & \text{Persistence} & \text{Consistency} & \text{Liveness} & \text{Scalability} & \text{Permissionless}  & \text{Slowly-adaptive}\\
        \midrule
                \text{\el}     &\cmark & \xmark & \cmark & \xmark & \cmark & \cmark\\

        \hline
                \text{\mx}     &\cmark & \cmark & \cmark & \xmark & \cmark & \cmark\\  
        \hline
                \text{\ol}         &\cmark & \cmark & \xmark & \cmark & \cmark  & \cmark \\ 
        \hline
                \text{\rc}      &\cmark & \cmark & \cmark & \cmark & \cmark & $\bm{\sim}$  \\ 
        \hline
                \text{\cs}     &\cmark & \cmark & \cmark & \cmark & \xmark & \xmark  \\ 
                
        \bottomrule
    \end{tabular}
    \label{tab:comparison}
    \vspace{-0.2cm}
\end{table*}

\subsection{\el}
\subsubsection*{Overview.}
\el is the first distributed blockchain sharding protocol introduced by Luu at al.~\cite{luu2016secure}. The protocol lies in the intersection of traditional BFT protocols and the Nakamoto consensus. 
The protocol is synchronous and proceeds in epochs. 
The setting is permissionless, and during each epoch the participants create valid identities by producing proof-of-work (PoW) solutions. 
The adversary is slowly-adaptive (as described in Section~\ref{sec:model}) and controls at most $f< \frac{n}{4}$ ($n$ valid identities in total) or $25\%$ of the  computational power of the system. 

At the beginning of each epoch, participants are partitioned into small shards (committees) of constant size $c$. The number of shards is $m=2^s$, where $s$ is a small constant such that $n=c \cdot 2^s$. A shard member contacts its directory committee to identify the other members of the same shard.
For each party, the directory committee consists of the first $c$ identities created in the epoch in the party's local view.
Transactions are randomly partitioned in disjoint sets based on the hash of the transaction input (in the UTXO model); hence each shard only processes a fraction of the total transactions in the system. The shard members execute a BFT protocol to validate the shard's transactions and then send the validated transactions to the final committee. The final committee consists of all members with a fixed $s$-bit shards identity, and is in charge of two operations: (i) computing and broadcasting the final block, which is a digital signature on the union of all valid received transactions\footnote{The final committee in \el broadcasts only the Merkle root for each block. However, this is asymptotically equivalent to including all transactions since the block size is constant. Furthermore, the final committee does not check if the received transactions are conflicting, but merely verifies the presence of signatures.} (via executing a BFT protocol), and (ii) generating and broadcasting a bounded exponential biased random string which is used as a public source of randomness in the next epoch (\eg\ for the PoW).

\subsubsection*{Summary of evaluation.}
We show that \el does not satisfy consistency due to its \texttt{CrossShard} protocol (as long as the workload does have cross-shard transactions). Additionally, \el does not satisfy scalability as all epoch-transition protocols (\eg, \texttt{Divide2Shards}, \texttt{CompactState}) are executed for every block (epoch in \el).
We highlight that \el does not satisfy scalability by design regardless the transaction distribution; that is, even with a few cross-shard transactions, \el maintains a global hash chain which is broadcasted to all the system's participants, and thus the scaling factor is constant at best (determined by the block size).

\subsection{\mx}
\subsubsection*{Overview.} 
Monoxide \cite{wang2019monoxide} is an asynchronous proof-of-work protocol, where the adversary controls at most $50\%$ of the computational power of the system.
The protocol uniformly partitions the space of user addresses into shards (zones) according to the first $k$ bits.
Every party is permanently assigned to a shard uniformly at random. Each shard employs the GHOST \cite{sompolinsky2015ghost} consensus protocol.

Participants are either full-nodes that verify and maintain the transaction ledgers, or miners investing computational power to solve PoW puzzles for profit in addition to being full-nodes. 
\mx introduces a new mining algorithm, called Chu-ko-nu, that enables miners to mine in parallel for all shards. 
The Chu-ko-nu algorithm aims to distribute the hashing power to protect individual shards from an adversarial takeover.
Successful miners include transactions in blocks. 
A block in \mx is divided into two parts: the chaining block that includes all metadata (Merkle root, nonce for PoW, etc.) creating the hash-chain, and the transaction-block that includes the list of transactions. All parties maintain the hash-chain of every shard in the system.

Furthermore, all parties maintain a distributed hash table for peer discovery and identifying parties in a specific shard. This way the parties of the same shard can identify each other and cross-shard transactions are sent directly to the destination shard.
Cross-shard transactions are validated in the shard of the payer and verified from the shard of the payee via a relay transaction and the hash-chain of the payer's shard.

\subsubsection*{Summary of evaluation.}
We show that \mx does not satisfy scalability because the state is not partitioned when security properties are satisfied. We observe that the lack of scalability stems from the protocol's mechanism to defend against adversaries in the PoW setting; hence it cannot scale even in an optimistic transaction distribution with no cross-shard transactions. 
% %

\subsection{\ol}
\subsubsection*{Overview.}
OmniLedger \cite{kokoris2017omniledger} proceeds in epochs, assumes a partially synchronous model within each epoch (to be responsive), synchronous communication channels between honest parties (with a large maximum delay), and a slowly-adaptive computationally-bounded adversary that can corrupt up to $f<n/4$ parties.

The protocol bootstraps using techniques from ByzCoin~\cite{kogias2016enhancing}. The core idea is that there is a global identity blockchain that is extended once per epoch with Sybil resistant proofs (proof-of-work, proof-of-stake, or proof-of-personhood~\cite{borge2017pop}) coupled with public keys. 
At the beginning of each epoch a sliding window mechanism is employed to define the eligible validators as the ones with identities in the last $W$ blocks, where $W$ depends on the adaptivity of the adversary. For our definition of slowly adaptive, we set $W=1$.
The UTXO space is partitioned uniformly at random into $m$ shards, each shard maintaining its own ledger.

At the beginning of each epoch, a new common random value is created via a distributed randomness generation (DRG) protocol. The DRG protocol employs verifiable random functions (VRF) to elect a leader who runs RandHound \cite{syta2017scalable} to create the random value.
The random value is used as a challenge for the next epoch's identity registration and as a seed to assigning identities of the current epoch into shards.

Once the participants for this epoch are assigned to shards and bootstrap their internal states, they start validating transactions and updating the shards' transaction ledgers by operating ByzCoinX, a modification of ByzCoin~\cite{kogias2016enhancing}.
When a transaction is cross-shard, a protocol that ensures the atomic operation of transactions across shards called \textit{Atomix} is employed. Atomix is a client-driven atomic commit protocol secure against Byzantine adversaries. 

\subsubsection*{Summary of evaluation.}
We prove that \ol maintains all properties but liveness. Specifically, \ol  uses checkpoints of the UTXO pool at the end of each epoch, but the state is not broadcasted to the network. Therefore, \ol is vulnerable to slowly adaptive adversaries that can corrupt a shard from the previous epoch before the new nodes of the shard bootstrap to the state during epoch transition. This attack violates the liveness property of the system. Nevertheless, simply adding a reliable broadcast step at the end of each epoch restores the liveness of \ol, as all other components satisfy liveness. The overhead of this step can be amortized over the rounds of the epoch hence scalability is also maintained.

\subsection{\rc}
\subsubsection*{Overview.}
RapidChain \cite{zamani2018rapidchain} is a synchronous protocol and proceeds in epochs. The adversary is slowly-adaptive, computationally-bounded and corrupts less than $1/3$ of the participants ($f<n/3$).

The protocol bootstraps via a committee election protocol that selects $O(\sqrt{n})$ parties -- the root group. The root group generates and distributes a sequence of random bits used to establish the reference committee. The reference committee consists of $O(\log n)$ parties, is re-elected at the end of each epoch, and is responsible for: (i) generating the randomness of the next epoch, (ii) validating the identities of participants for the next epoch from the PoW puzzle, and (iii) reconfiguring the shards from one epoch to the next (to protect against single shard takeover attacks).

The parties are divided into shards of size $O(\log n)$ (committees). Each shard handles a fraction of the transactions, assigned based on the prefix of the transaction ID. Transactions are sent by external users to an arbitrary number of active (for this epoch) parties. The parties then use an inter-shard routing scheme (based on Kademlia~\cite{maymounkov2002kademlia}) to send the transactions to the input and output shards, \ie, the shards handling the inputs and outputs of a transaction, respectively.

To process cross-shard transactions, the leader of the output shard creates an additional transaction for every different input shard. Then the leader sends (via the inter-shard routing scheme) these transactions to the corresponding input shards for validation. 
% To process cross-shard transactions, the leader of the output shard creates one additional transaction for every different input shard which the leader sends (via the inter-shard routing scheme) to the input shard for validation. 
To validate transactions (\ie, a block), each shard runs a variant of the synchronous consensus of Ren et al.~\cite{ren2017practical} and thus tolerates $1/2$ Byzantine parties. 

At the end of each epoch, the shards are reconfigured according to the participants registered in the new reference block. Specifically, \rc uses a bounded version of Cuckoo rule \cite{sen2012commensal}; the reconfiguration protocol adds a new party to a shard uniformly at random, and also moves a constant number of parties from each shard and assigns them to other shards uniformly at random. 


\subsubsection*{Summary of evaluation.}
 We prove \rc maintains a robust sharded ledger but only under a weaker model than the one defined in Section~\ref{sec:model}. 
Specifically, the protocol only allows a constant number of parties to join or leave and the adversary can at most corrupt a constant number of additional parties with each epoch transition. 
\com{
Moreover, the security of the protocol is maintained for a limited amount of time since the epoch transition is secure as long as the number of epochs is asymptotically less than polynomial to the number of parties.}
Another shortcoming of \rc is the synchronous consensus mechanism it employs. 
In case of temporary loss of synchrony in the network, the consensus of cross-shard transactions is vulnerable, hence consistency might break~\cite{zamani2018rapidchain}.
However, most of these drawbacks can be addressed with simple solutions, such as changing the consensus protocol (trade-off performance with security), replacing the epoch transition process with one similar to (fixed) \ol, etc. 
Although \ol (with the proposed fix) maintains a robust sharded ledger in a stronger model (as defined in Section~\ref{sec:model}), \rc introduces practical speedups on specific components of the system. These improvements are not asymptotically important -- and thus not captured by our framework -- but might be significant for the performance of  deployed sharding protocols.

\subsection{\cs}
\subsubsection*{Overview.}
\cs is a sharding protocol introduced by Al-Bassam et al.~\cite{al2018chainspace} that operates in the permissioned setting. 
The main innovation of \cs is on the application layer. Specifically, \cs presents a sharded, UTXO-based distributed ledger that supports smart contracts. Furthermore, limited privacy is enabled by offloading computation to the clients, who need to only publicly provide zero-knowledge proofs that their computation is correct.
\cs focuses on specific aspects of sharding; epoch transition or reconfiguration of the protocol is not addressed.
Nevertheless, the cross-shard communication protocol, namely S-BAC, is of interest as a building block to secure sharding. 

\subsubsection*{Summary of evaluation.}
We also include \cs in the comparison of sharding protocols, which maintains a robust sharded transaction ledger but only in the permissioned setting against a static adversary. 
\cs could be secure in our model in the permissioned setting if it adopts \ol's epoch transition protocols and the proposed fix for data availability in the verifiable compaction of state.
We omit the security proofs for \cs since they are either included in \cite{al2018chainspace} or are similar to \ol.
We include in the evaluation the ``permissionless'' and ``slowly-adaptive'' property, in addition to the security and efficiency properties, namely persistence, consistency, liveness and scalability.

Lastly, we note that the cross-shard communication protocols of some of these sharding systems suffer from replay attacks~\cite{sonnino2019replay}. In our analysis, we consider the fixes proposed in~\cite{sonnino2019replay}.




% We first show that \el does not satisfy consistency due to its \texttt{CrossShard} protocol (as long as the workload does have cross-shard transactions). Additionally, \el does not satisfy scalability as all epoch-transition protocols (\eg, \texttt{Divide2Shards}, \texttt{CompactState}) are executed for every block (epoch in \el).
% We highlight that \el does not satisfy scalability by design regardless the transaction distribution; that is, even with a few cross-shard transactions, \el maintains a global hash chain which is broadcast to all the system's participants, and thus the scaling factor is constant at best (determined by the block size).

% We then show that \mx does not satisfy scalability because the state is not partitioned when security properties are satisfied. We observe that the lack of scalability stems from the protocol's mechanism to defend against adversaries in the PoW setting; hence it cannot scale even in an optimistic transaction distribution with no cross-shard transactions. 
% %

% Third, we prove that \ol maintains all properties but liveness. Specifically, \ol  uses checkpoints of the UTXO pool at the end of each epoch, but the state is not broadcast to the network. Therefore, \ol is vulnerable to slowly adaptive adversaries that can corrupt a shard from the previous epoch before the new nodes of the shard bootstrap to the state during epoch transition. This attack violates the liveness property of the system. Nevertheless, simply adding a reliable broadcast step at the end of each epoch restores the liveness of \ol, as all other components satisfy liveness. The overhead of this step can be amortized over the rounds of the epoch hence scalability is also maintained.

% Fourth, we prove \rc maintains a robust sharded ledger but only under a weaker model than the one defined in Section~\ref{sec:model}. 
% Specifically, the protocol only allows a constant number of parties to join or leave and the adversary can at most corrupt a constant number of additional parties with each epoch transition. 
% \com{
% Moreover, the security of the protocol is maintained for a limited amount of time since the epoch transition is secure as long as the number of epochs is asymptotically less than polynomial to the number of parties.}
% Another shortcoming of \rc is the synchronous consensus mechanism it employs. 
% In case of temporary loss of synchrony in the network, the consensus of cross-shard transactions is vulnerable, hence consistency might break~\cite{zamani2018rapidchain}.
% However, most of these drawbacks can be addressed with simple solutions, such as changing the consensus protocol (trade-off performance with security), replacing the epoch transition process with one similar to (fixed) \ol, etc. 
% Although \ol (with the proposed fix) maintains a robust sharded ledger in a stronger model (as defined in Section~\ref{sec:model}), \rc introduces practical speedups on specific components of the system. These improvements are not asymptotically important -- and thus not captured by our framework -- but might be significant for the performance of  deployed sharding protocols.

% Finally, we include \cs in the comparison of sharding protocols, which maintains a robust sharded transaction ledger but only in the permissioned setting against a static adversary. 
% \cs could be secure in our model in the permissioned setting if it adopts \ol's epoch transition protocols and the proposed fix for data availability in the verifiable compaction of state.
% We omit the security proofs for \cs since they are either included in \cite{al2018chainspace} or are similar to \ol.
% We include in the evaluation the ``permissionless'' and ``slowly-adaptive'' property, in addition to the security and efficiency properties, namely persistence, consistency, liveness and scalability.

% Lastly, we note that the cross-shard communication protocols of some of these sharding systems suffer from replay attacks~\cite{sonnino2019replay}. In our analysis, we consider the fixes proposed in~\cite{sonnino2019replay}.
 



==> 6related.tex <==
 %-------------------RELATED WORK-------------------------
\section{Related work}\todo{rewrite}
The Bitcoin backbone protocol~\cite{garay2015bitcoin} was the first to formally define and prove a blockchain protocol, specifically Bitcoin, in a PoW setting. Later, Pass et al.~\cite{pass2017analysis} showed that there is no PoW protocol that can be robust under asynchrony. 
With Ouroboros~\cite{kiayias2017ouroboros} Kiayias et al.\ extended the ideas of backbone to the Proof-of-Stake (PoS) setting, where they showed that it is possible to have a robust transaction ledger in a semi-synchronous environment as well~\cite{david2018ouroboros}. 
Our work is also extending the backbone framework to define a robust sharded ledger. We also analyze state-of-the-art sharding protocols under our framework.

Recently, a few systemization of knowledge papers on sharding~\cite{wang2019sharding}, consensus~\cite{bano2017consensus} and cross-shard communication~\cite{zamyatin2019sok} which have also discussed part of sharding, have emerged. 
Unlike these, our focus is not a exhaustive list of existing protocols. Instead, we formally define what a robust sharded ledger is, evaluate existing sharding protocols under this lens, by either proving or disproving their claims in our framework, and provide a roadmap to robust sharding.

 \paragraph{Application.}
 Although we restrict our evaluation to the most impactful (so far) sharding proposals, we stress that the power of our framework and the bounds we provide are not limited to these works. For instance, we observe that Chainweb~\cite{martino2018chainweb}, a recently deployed sharding proposal, is not scalable -- as it claims -- because it violates Theorem~\ref{thm:scale-SPV}.
 We believe our framework is general enough to cover most sharding approaches, and we aspire it will be established as a tool for proving security of future sharding protocols.

\paragraph{Multi-consensus vs uni-consensus.}
 In our study, we assumed all shards run consensus to ensure the transaction validity (multi-consensus). A different approach that was recently proposed~\cite{rana2020free2shard,al2019lazyledger}, the so-called uni-consensus, suggests a system design where the transaction order, and thus the transaction validity, is established through a main hash-chain that contains the compressed information for all shards. 
 To achieve almost linear scaling, breaking the impossibility result of Theorem~\ref{thm:adaptive}, \cite{rana2020free2shard} propose dynamically adjustable block size, proportional to the number of nodes in the network.
%  Such a proposition is indeed useful because it implies that a protocol can scale almost linearly to the number of nodes simply via the linear compression of the information.
%  
 We consider this approach outside the realm of our study, since \textit{the growth of such a system inevitably leads to increased resource requirements} (\eg, bandwidth of each node). This holds because the information compressed in the hash-chain must be at least linear to the number of nodes in the network for such a system to scale. But this means that the block size is at least linear to the number of nodes in the network, which in turn implies that the bandwidth of each node will grow proportionally to the growth of the system. This contradicts the definition of sharding and we therefore believe such systems fall under the study of performance optimizations on the consensus layer of blockchains, \eg, \cite{androulaki18hyperledger,eyal2016bitcoinng,stathakopoulou2019mir,avarikioti2020fnfbft}. 


==> 7conclusion.tex <==
\section{Conclusion}

In this paper we provided the first complete analysis of sharded blockchains to enable ``apples-to-apples'' comparison. To this end we first proved several impossibility results and lower bounds on the security and scalability of sharded distributed ledgers. Equipped with the knowledge of these limitations we formalized Divide \& Scale, a protocol composition that maintains a robust sharded distributed ledger. Finally, we investigated existing sharding proposals and showed that their lack of formal treatment leads to all of them being subpar (or clearly broken) to Divide \& Scale.
